Learning Consistent Temporal Grounding between Related Tasks in Sports Coaching

Video-LLMs often attend to irrelevant frames, which is especially detrimental for sports coaching tasks requiring precise temporal grounding. Yet obtaining frame-level supervision is challenging: expensive to collect from humans and unreliable from other models. We improve temporal grounding without additional annotations by exploiting the observation that related tasks, such as generation and verification, must attend to the same frames. We enforce this via a self-consistency objective over select visual attention maps of tightly-related tasks. Using VidDiffBench, which provides ground-truth keyframe annotations, we first validate that attention misallocation is a significant bottleneck. We then show that training with our objective yields gains of +3.0%, +14.1% accuracy and +0.9 BERTScore over supervised finetuning across three sports coaching tasks: Exact, FitnessQA, and ExpertAF, even surpassing closed-source models.

==> dump.tex <==
%move to rel works In \cite{zhang2025cross}, it is found that early layers in MLLMs propogate visual information to the text tokens, and then in the mid-level layers tokens that correspond to relevant objects in the image are attended to by the object mentions in the questions. 

% they have shown that attention patterns from particular layers can be used to ``zoom in'' on relevants aspects of an image \cite{zhang2025mllms}, [citation] or visual attention sinks, have only been limited to llava \cite{liu2023llava} and images. While \cite{chen2025spatial} sharpens or flattens based on answer confidence, we find no correlation for videos. This could be because the model...

==> tables/ablation_k_hyperparam.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lcc}
\toprule
\textbf{$K$} & \textbf{Exact} \\
\midrule
5   & \textbf{87.5}  \\
10 & 84.5  \\
15 & 80.0 \\
25 & 81.5 \\
32 & 63.5  \\
\bottomrule
\end{tabular}
\caption{Ablation over the number of Top-$K$ heads selected per pathway via Visual Non-Sink Ratio. All other components are fixed.}
\label{tab:k_ablation}
\end{table}
